A Comparison of the Baryonic Tully-Fisher Relation in MaNGA and IllustrisTNG

We compare an observed Baryonic Tully-Fisher Relation (BTFR) from the Mapping Nearby Galaxies at Apache Point Observatory (MaNGA) and HI-MaNGA surveys to a simulated BTFR from the cosmological magnetohydrodynamical simulation IllustrisTNG. To do so, we calibrate the BTFR of the local universe using 377 galaxies from the MaNGA and HI-MaNGA surveys, and perform mock 21 cm observations of matching galaxies from IllustrisTNG. The mock observations are used to ensure that the comparison with the observed galaxies is fair since it has identical measurement algorithms, observational limitations, biases and uncertainties. For comparison, we also calculate the BTFR for the simulation without mock observations, and demonstrate how mock observations are necessary to fairly and consistently compare between observational and theoretical data. We report a MaNGA BTFR of log$_{10} (M_{ \rm Bary}/M_\odot)= (2.97 \pm 0.18)$ log$_{10} V_{ \rm Rot} + (4.04 \pm 0.41)\,\log_{10}{M_{\odot}}$ and an IllustrisTNG BTFR of log$_{10} (M_{ \rm Bary}/M_\odot) = (2.94 \pm 0.23$) log$_{10} V_{ \rm Rot} + (4.15 \pm 0.44)\,\log_{10}{M_{\odot}}$. Thus, MaNGA and IllustrisTNG produce BTFRs that agree within uncertainties, demonstrating that IllustrisTNG has created a galaxy population that obeys the observed relationship between mass and rotation velocity in the observed universe.

==> sparecontent.tex <==
\begin{table*}
 \centering
 \begin{tabular}{l|c|c|c|c|c}
 \hline
 & MaNGA  & IllustrisTNG & IllustrisTNG using  & MaNGA  & IllustrisTNG \\
 & with $\Delta t$ &  with $\Delta t$ &  $V_{\rm MAX}$ directly & without $\Delta t$ &  without $\Delta t$ \\
 \hline 
 \hline
  \textcolor{red}{$V_{\rm 50,Rot}$} Forward slope [Log($M_\odot$)/Log(\textcolor{red}{km\,s$^{-1}$}] &  2.59 $\pm$ 0.09 & 2.52 $\pm$ 0.13 & 3.48 $\pm$ 0.07 & 2.74 $\pm$ 0.10 & 2.48 $\pm$ 0.20 \\
 \textcolor{red}{$V_{\rm 50,Rot}$} Inverse slope {[Log($M_\odot$)/Log(\textcolor{red}{km\,s$^{-1}$})]} & 3.45 $\pm$ 0.16 & 3.57 $\pm$ 0.28 & 3.83 $\pm$ 0.07 & 3.57 $\pm$ 0.17 & 3.74 $\pm$ 0.31 \\
 \textcolor{red}{$V_{\rm 50,Rot}$} Bisector slope [Log($M_\odot$)/Log(\textcolor{red}{km\,s$^{-1}$}] & 2.97 $\pm$ 0.18 & 2.97 $\pm$ 0.22 & 3.65 $\pm$ 0.06 & 3.11 $\pm$ 0.19 & 2.97 $\pm$ 0.29 \\
 \hline
 \textcolor{red}{$V_{\rm 50,Rot}$} Forward intercept [Log($M_\odot$)] & 4.76 $\pm$ 0.19 & 4.91 $\pm$ 0.27 & 2.60 $\pm$ 0.14 & 4.40 $\pm$ 0.21 & 4.96 $\pm$ 0.42 \\
 \textcolor{red}{$V_{\rm 50,Rot}$} Inverse intercept [Log($M_\odot$)] & 2.95 $\pm$ 0.33 & 2.75 $\pm$ 0.57 & 1.89 $\pm$ 0.15 & 2.64 $\pm$ 0.36 & 2.36 $\pm$ 0.63 \\ 
 \textcolor{red}{$V_{\rm 50,Rot}$} Bisector intercept [Log($M_\odot$)] & 4.05 $\pm$ 0.40 & 4.12 $\pm$ 0.44 & 2.25 $\pm$ 0.12 & 3.70 $\pm$ 0.40 & 4.12 $\pm$ 0.50 \\
 %\hline
 %\textcolor{red}{$V_{\rm 20,Rot}$ Forward slope [Log($M_\odot$)/Log(km\,s$^{-1}$)]} &  \textcolor{red}{2.50 $\pm$ 0.17} & \textcolor{red}{2.57 $\pm$ 0.10} & \textcolor{red}{N/A}  & \textcolor{red}{N/A} & N/A \\ 
 \hline
 \end{tabular}
  \caption{Our various BTFR fits, demonstrating the agreement between the BTFR from MaNGA and IllustrisTNG when employing the mock observations to ensure a fair comparison between the observations and simulation, but that they do not agree without the mock observations. We also demonstrate that removing the turbulence (velocity dispersion) correction has minimal effect on the MaNGA and IllustrisTNG BTFR. Consequently, this correction does not account for our shallow slopes compared with the literature. \textcolor{red}{I started modifying this table but then stopped because I'm not sure if it is necessary since it seems to have the exact same information as Table 3 (minus the ``IllustrisTNG using $V_{\rm MAX}$ directly" column)}}
 \label{tab:BTFRfits}
\end{table*}


% \hline
% \hline
% \textcolor{red}{MaNGA: $V_{\rm 20,Rot}$ vs. $M_{\rm Bary}$} & \textcolor{red}{Yes} & \textcolor{red}{Yes} & \textcolor{red}{368} & \textcolor{red}{43} & \textcolor{red}{325} & \textcolor{red}{2.65 $\pm$ 0.14} & \textcolor{red}{4.49 $\pm$ 0.30} \\
% \textcolor{red}{MaNGA: $M_{\rm Bary}$ vs. $V_{\rm 20,Rot}$} & \textcolor{red}{Yes} & \textcolor{red}{Yes} & \textcolor{red}{368} & \textcolor{red}{5} & \textcolor{red}{363} & \textcolor{red}{3.75 $\pm$ 0.19} & \textcolor{red}{2.12 $\pm$ 0.40}\\
% \textcolor{red}{MaNGA: $V_{\rm 20,Rot}$ Bisector} & \textcolor{red}{Yes} & \textcolor{red}{Yes} & \textcolor{red}{368} & \textcolor{red}{43} & \textcolor{red}{325} & \textcolor{red}{3.11 $\pm$ 0.18} & \textcolor{red}{3.52 $\pm$ 0.38} \\
% \hline
% \textcolor{red}{IllustrisTNG: $V_{\rm 20,Rot}$ vs. $M_{\rm Bary}$} & \textcolor{red}{Yes} & \textcolor{red}{Yes} & \textcolor{red}{330} & \textcolor{red}{34} & \textcolor{red}{296} & \textcolor{red}{2.55 $\pm$ 0.11} & \textcolor{red}{4.89 $\pm$ 0.22} \\
% \textcolor{red}{IllustrisTNG: $M_{\rm Bary}$ vs. $V_{\rm 20,Rot}$} & \textcolor{red}{Yes} & \textcolor{red}{Yes} & \textcolor{red}{330} & \textcolor{red}{6} & \textcolor{red}{324} & \textcolor{red}{3.93 $\pm$ 0.31} & \textcolor{red}{1.99 $\pm$ 0.64} \\
% \textcolor{red}{IllustrisTNG: $V_{\rm 20,Rot}$ Bisector} & \textcolor{red}{Yes} & \textcolor{red}{Yes} & \textcolor{red}{330} & \textcolor{red}{35} & \textcolor{red}{295} & \textcolor{red}{3.11 $\pm$ 0.20} & \textcolor{red}{3.73 $\pm$ 0.41} \\
% \textcolor{red}{MaNGA: $V_{\rm 20,Rot}$ vs. $M_{\rm Bary}$} & \textcolor{red}{No} & \textcolor{red}{No} & \textcolor{red}{377} & \textcolor{red}{36} & \textcolor{red}{341} & \textcolor{red}{2.53 $\pm$ 0.19} & \textcolor{red}{4.71 $\pm$ 0.42} \\
% \textcolor{red}{MaNGA: $M_{\rm Bary}$ vs. $V_{\rm 20,Rot}$} & \textcolor{red}{No} & \textcolor{red}{No} & \textcolor{red}{377} & \textcolor{red}{5} & \textcolor{red}{372} & \textcolor{red}{3.84 $\pm$ 0.19} & \textcolor{red}{1.89 $\pm$ 0.42}\\
% \textcolor{red}{MaNGA: $V_{\rm 20,Rot}$ Bisector} & \textcolor{red}{No} & \textcolor{red}{No} & \textcolor{red}{377} & \textcolor{red}{36} & \textcolor{red}{341} & \textcolor{red}{3.06 $\pm$ 0.17} & \textcolor{red}{3.58 $\pm$ 0.37} \\
% \hline
% \textcolor{red}{IllustrisTNG: $V_{\rm 20,Rot}$ vs. $M_{\rm Bary}$} & \textcolor{red}{No} & \textcolor{red}{No} & \textcolor{red}{377} & \textcolor{red}{36} & \textcolor{red}{341} & \textcolor{red}{2.46 $\pm$ 0.10} & \textcolor{red}{5.13 $\pm$ 0.22} \\
% \textcolor{red}{IllustrisTNG: $M_{\rm Bary}$ vs. $V_{\rm 20,Rot}$} & \textcolor{red}{No} & \textcolor{red}{No} & \textcolor{red}{377} & \textcolor{red}{9} & \textcolor{red}{368} & \textcolor{red}{3.81 $\pm$ 0.21} & \textcolor{red}{2.51 $\pm$ 0.44} \\
% \textcolor{red}{IllustrisTNG: $V_{\rm 20,Rot}$ Bisector} & \textcolor{red}{No} & \textcolor{red}{No} & \textcolor{red}{377} & \textcolor{red}{36} & \textcolor{red}{341} & \textcolor{red}{2.97
% $\pm$ 0.15} & \textcolor{red}{4.05 $\pm$ 0.24} \\
% \hline
% \hline
% \hline
% \textcolor{red}{MaNGA: $V_{\rm 50,Rot}$ vs. $M_{\rm Bary}$} & \textcolor{red}{No} & \textcolor{red}{Yes} & \textcolor{red}{368} & \textcolor{red}{85} & \textcolor{red}{283} & \textcolor{red}{2.74 $\pm$ 0.09} & \textcolor{red}{4.41 $\pm$ 0.20} \\
% \textcolor{red}{MaNGA: $M_{\rm Bary}$ vs. $V_{\rm 50,Rot}$} & \textcolor{red}{No} & \textcolor{red}{Yes} & \textcolor{red}{368} & \textcolor{red}{7} & \textcolor{red}{361} & \textcolor{red}{3.59 $\pm$ 0.17} & \textcolor{red}{2.62 $\pm$ 0.36}\\
% \textcolor{red}{MaNGA: $V_{\rm 50,Rot}$ Bisector} & \textcolor{red}{No} & \textcolor{red}{Yes} & \textcolor{red}{368} & \textcolor{red}{85} & \textcolor{red}{283} & \textcolor{red}{3.12 $\pm$ 0.19} & \textcolor{red}{3.69 $\pm$ 0.41} \\
% \hline
% \textcolor{red}{IllustrisTNG: $V_{\rm 50,Rot}$ vs. $M_{\rm Bary}$} & \textcolor{red}{No} & \textcolor{red}{Yes} & \textcolor{red}{330} & \textcolor{red}{69} & \textcolor{red}{261} & \textcolor{red}{2.78 $\pm$ 0.16} & \textcolor{red}{4.28 $\pm$ 0.34} \\
% \textcolor{red}{IllustrisTNG: $M_{\rm Bary}$ vs. $V_{\rm 50,Rot}$} & \textcolor{red}{No} & \textcolor{red}{Yes} & \textcolor{red}{330} & \textcolor{red}{0} & \textcolor{red}{330} & \textcolor{red}{3.85 $\pm$ 0.32} & \textcolor{red}{2.11 $\pm$ 0.66} \\
% \textcolor{red}{IllustrisTNG: $V_{\rm 50,Rot}$ Bisector} & \textcolor{red}{No} & \textcolor{red}{Yes} & \textcolor{red}{330} & \textcolor{red}{69} & \textcolor{red}{261} & \textcolor{red}{3.24 $\pm$ 0.26} & \textcolor{red}{4.12 $\pm$ 0.55} \\
% \hline
% \hline
% \textcolor{red}{MaNGA: $V_{\rm 20,Rot}$ vs. $M_{\rm Bary}$} & \textcolor{red}{No} & \textcolor{red}{Yes} & \textcolor{red}{368} & \textcolor{red}{40} & \textcolor{red}{328} & \textcolor{red}{2.68 $\pm$ 0.16} & \textcolor{red}{4.38 $\pm$ 0.34} \\
% \textcolor{red}{MaNGA: $M_{\rm Bary}$ vs. $V_{\rm 20,Rot}$} & \textcolor{red}{No} & \textcolor{red}{Yes} & \textcolor{red}{368} & \textcolor{red}{5} & \textcolor{red}{363} & \textcolor{red}{3.86 $\pm$ 0.20} & \textcolor{red}{1.83 $\pm$ 0.44}\\
% \textcolor{red}{MaNGA: $V_{\rm 20,Rot}$ Bisector} & \textcolor{red}{No} & \textcolor{red}{Yes} & \textcolor{red}{368} & \textcolor{red}{40} & \textcolor{red}{328} & \textcolor{red}{3.18 $\pm$ 0.17} & \textcolor{red}{3.33 $\pm$ 0.39} \\
% \hline
% \textcolor{red}{IllustrisTNG: $V_{\rm 20,Rot}$ vs. $M_{\rm Bary}$} & \textcolor{red}{Yes} & \textcolor{red}{No} & \textcolor{red}{330} & \textcolor{red}{30} & \textcolor{red}{300} & \textcolor{red}{2.64 $\pm$ 0.11} & \textcolor{red}{4.89 $\pm$ 0.22} \\
% \textcolor{red}{IllustrisTNG: $M_{\rm Bary}$ vs. $V_{\rm 20,Rot}$} & \textcolor{red}{No} & \textcolor{red}{Yes} & \textcolor{red}{330} & \textcolor{red}{7} & \textcolor{red}{323} & \textcolor{red}{4.06 $\pm$ 0.35} & \textcolor{red}{1.76 $\pm$ 0.66} \\
% \textcolor{red}{IllustrisTNG: $V_{\rm 20,Rot}$ Bisector} & \textcolor{red}{No} & \textcolor{red}{Yes} & \textcolor{red}{330} & \textcolor{red}{30} & \textcolor{red}{300} & \textcolor{red}{3.22 $\pm$ 0.20} & \textcolor{red}{3.56 $\pm$ 0.41} \\

%\textcolor{red}{IllustrisTNG: $V_{\rm Max}$ vs. $M_{\rm Bary}$} & \textcolor{red}{N/A} & \textcolor{red}{Yes} & \textcolor{red}{330} & \textcolor{red}{0} & \textcolor{red}{330} & \textcolor{red}{3.53 $\pm$ 0.07} & \textcolor{red}{2.49 $\pm$ 0.15} \\
%\textcolor{red}{IllustrisTNG: $M_{\rm Bary}$ vs. $V_{\rm Max}$} & \textcolor{red}{N/A} & \textcolor{red}{Yes} & \textcolor{red}{330} & \textcolor{red}{0} & \textcolor{red}{330} & \textcolor{red}{3.92 $\pm$ 0.09} & \textcolor{red}{1.67 $\pm$ 0.20} \\ 
% \textcolor{red}{IllustrisTNG: $V_{\rm Max}$ Bisector} & \textcolor{red}{N/A} & \textcolor{red}{Yes} & \textcolor{red}{330} & \textcolor{red}{0} & \textcolor{red}{330} & \textcolor{red}{3.72 $\pm$ 0.13} & \textcolor{red}{2.09 $\pm$ 0.27} \\
